Low-Energy Line Codes for On-Chip Networks

Energy is a primary constraint in processor design, and much of that energy is consumed in on-chip communication. Communication can be intra-core (e.g., from a register file to an ALU) or inter-core (e.g., over the on-chip network). In this paper, we use the on-chip network (OCN) as a case study for saving on-chip communication energy. We have identified a new way to reduce the OCN's link energy consumption by using line coding, a longstanding technique in information theory. Our line codes, called Low-Energy Line Codes (LELCs), reduce energy by reducing the frequency of voltage transitions of the links, and they achieve a range of energy/performance trade-offs.

==> tables.tex <==
\usepackage{colortbl}
\usepackage[table]{xcolor}
\usepackage{wrapfig}


\subsection{Appendix}
\subsubsection{Input Characteristics} \label{app_b3} \hfill

\begin{table} [!htbp]
\begin{minipage}[h]{0.6\linewidth}
\centering
\includegraphics[trim={0in 0.3in 0in 0in},width=4in, height=1.5in]{blackscholes.png}
\captionof{figure}{Blackscholes benchmark 6-tuple vector input statistics.}
\label{patterns}
\vspace{-1em}
\end{minipage}
\hspace{0.2em}
\begin{minipage}[h]{0.4\linewidth}
\centering
\includegraphics[trim={0in 0.3in 0in 0in},clip,width=2.5in,height=1.5in]{blackscholes_w.png}
\captionof{figure}{Blackscholes benchmark 6-tuple vector input statistics according to weight.}
\label{patterns}
\vspace{-1em}
\end{minipage}\hfill
\end{table}

\begin{table} [!htbp]
\begin{minipage}[h]{0.6\linewidth}
\centering
\includegraphics[trim={0in 0.3in 0in 0in},width=4in, height=1.5in]{fluidanimate.png}
\captionof{figure}{Fluidanimate benchmark 6-tuple vector input statistics.}
\label{patterns}
\vspace{-1em}
\end{minipage}
\hspace{0.2em}
\begin{minipage}[h]{0.4\linewidth}
\centering
\includegraphics[trim={0in 0.3in 0in 0in},clip,width=2.5in,height=1.5in]{fluidanimate_w.png}
\captionof{figure}{Fluidanimate benchmark 6-tuple vector input statistics according to weight.}
\label{patterns}
\vspace{-1em}
\end{minipage}\hfill

\end{table}


\subsubsection{Table Illustrating the Performance of all Coding Schemes} \label{app_c1} \hfill

\begin{figure}[H]
  \centering
    \captionof{table}{Performance (Rate and Percentage Power Reduction) of all the codes we designed, color coded based on coding scheme, on benchamrks; Fluidanimate, Blackscholes, and Canneal .}
    \label{ftable}
    \includegraphics[trim={0in 0in 0in 0in},heght=0.95\textheight]{tablo2.JPG}
\end{figure}

\newpage
\subsubsection{Trees Designed Considering Benchmark Data} \label{app_c2} \hfill 
\hfill


\begin{table} [!htbp]
\begin{minipage}[h]{0.5\linewidth}
\centering
\includegraphics[trim={0in 0in 0in 0in},width=3in]{tree2.jpg}
\captionof{figure}{Tree Option 2: Focuses on compression of all $1$s stream.}
\label{tree2}
\vspace{-1em}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.5\linewidth}
\centering
\vspace{9em}
\includegraphics[trim={0in 0in 0in 0in},clip,width=3in]{tree3.jpg}
\captionof{figure}{Tree Option 3: Focuses on minimizing rate loss in the majority of the distribution.}
\label{tree3}
\end{minipage}\hfill
\end{table}

\hfill\hfill

\begin{table} [!htbp]
\begin{minipage}[h]{0.5\linewidth}
\centering
\vspace{2em}
\includegraphics[trim={0in 0in 0in 0in},width=3in]{tree4.jpg}
\vspace{0.5em}
\captionof{figure}{Tree Option 4: Focuses on more compression all $1$s stream, while keeping rate loss in distribution less (combination of trees 2 and 3).}
\label{tree4}
\vspace{-1em}
\end{minipage}
\hspace{1em}
\begin{minipage}[h]{0.5\linewidth}
\centering
\includegraphics[trim={0in 0in 0in 0in},clip,width=3in]{tree5.jpg}
\captionof{figure}{Tree Option 5: Focuses no rate loss in all $0$s stream and compression all $1$s at the same time.}
\label{tree5}
\vspace{-1em}
\end{minipage}\hfill
\end{table}


\newpage
\subsubsection{Coding Scheme with LUT Targeting Input Statistics} \label{app_c3} \hfill 
\hfill

\begin{table}[H]
\caption{Analysis of codes targeting input statistics, before and after forcing the constraint of "there does not exist any codeword with increased number of $1$s" on the LUT.}
\centering
\scalebox{0.85}
{
\begin{tabular}{c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c}
    \hline
     & & Rate & PR\% & \shortstack{Output \\ Length} & \shortstack{Output \\ $1$ Count} & \shortstack{Total change in \\ Number(\#) of $1$s} & \shortstack{LOSS in \\ \# of $1$s} & \shortstack{\% codeword \\ count with loss}  & \shortstack{Avg. change in \\ \# of $1$s} \\ \hline
    Blackscholes & \shortstack{Before \\ Constraint} & 0.89 & 47\% & 36288 & 6195 & $-5597$ & $+367$ & $\frac{329}{4032}\times100 \approx 8\%$ & $-1.39$ \\\arrayrulecolor{white}\hline
     & \shortstack{After \\ Constraint} & 0.89 & 34\% & 36288 & 7756 & $-4036$ & 0 & 0 & $-1.00$ \\ \arrayrulecolor{black}\hline
    Canneal & \shortstack{Before \\ Constraint} & 0.89 & 44\% & 4911354 & 842503 & $-663333$ & $+57334$ & $\frac{56244}{545706}\times100 \approx 10\%$ & $-1.22$ \\\arrayrulecolor{white}\hline
     & \shortstack{After \\ Constraint} & 0.89 & 35\% & 4911354 & 972115 & $-533721$ & 0 & 0 & $-0.98$ \\ \arrayrulecolor{black}\hline
    Fluidanimate & \shortstack{Before \\ Constraint} & 0.89 & 43\% & 51840 & 6091 & $-4628$ & $+288$ & $\frac{269}{5760}\times100 \approx 4.7\%$ & $-0.80$ \\\arrayrulecolor{white}\hline
     & \shortstack{After \\ Constraint} & 0.89 & 31\% & 51840 & 7421 & $-3298$ & 0 & 0 & $-0.57$ \\ \arrayrulecolor{black}\hline
\end{tabular}}
\label{table_ctis}
\end{table}



\begin{table}[H]
\caption{Performance on all benchmarks using LUT designed for a specific benchmark.}
\centering
\scalebox{0.85}
{
\begin{tabular}{c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c}
    \hline
     Performance on & \shortstack{Look-up table of \\ Blackscholes} & \shortstack{Look-up table of \\ Canneal} & \shortstack{Look-up table of \\ Fluidanimate}  \\ \hline
    Blackscholes & \cellcolor{yellow!25}47.46\% & 37.57\% & 34.56\%  \\ \arrayrulecolor{black}\hline
    Canneal &  35.11\% & \cellcolor{yellow!25}44.05\% & 37.74\%  \\ \arrayrulecolor{black}\hline
    Fluidanimate & 28.92\% & 34.81\% & \cellcolor{yellow!25}43.18\%  \\ \arrayrulecolor{black}\hline
\end{tabular}}
\label{table_lut}
\end{table}

\vspace{3em}

\subsubsection{Dynamic Packet Processor Library Results} \label{app_c4} \hfill 

\begin{table}[H]
\caption{Percentage time spent on low rate and high rate code and corresponding percentage increase in number of cycles with respect to different utilization markers on Blackscholes benchmark.}
\centering
\scalebox{0.85}
{
\begin{tabular}{ | c | c | c | c | c |}
    \hline
    \shortstack{\% Utilization \\ Marker} & \shortstack{\% Time Spent at \\ High Rate Code \\ ($R=1$)} & \shortstack{\% Time Spent at \\ Low Rate Code \\ ($R=0.75$)} & \shortstack{Number \\ of Cycles} & \shortstack{\% Increase in \\ Number of Cycles \\ (baseline = $7.732\times10^8$)} \\ \hline 
    5.50\% & 70.2\% & 29.8\% & $7.791\times10^8$ & 0.76\% \\ \hline
    6.18\% & 50.0\% & 50.0\% & $8.048\times10^8$ & 4.09\% \\ \hline
    6.50\% & 36.1\% & 63.9\% & $8.199\times10^8$ & 6.04\% \\ \hline
    7.00\% & 33.5\% & 66.5\% & $8.210\times10^8$ & 6.18\%  \\ \hline
\end{tabular}}
\label{table_dp}
\end{table}
